Equivalence Between SE(3) Equivariant Networks via Steerable Kernels and Group Convolution

A wide range of techniques have been proposed in recent years for designing neural networks for 3D data that are equivariant under rotation and translation of the input. Most approaches for equivariance under the Euclidean group $\mathrm{SE}(3)$ of rotations and translations fall within one of the two major categories. The first category consists of methods that use $\mathrm{SE}(3)$-convolution which generalizes classical $\mathbb{R}^3$-convolution on signals over $\mathrm{SE}(3)$. Alternatively, it is possible to use \textit{steerable convolution} which achieves $\mathrm{SE}(3)$-equivariance by imposing constraints on $\mathbb{R}^3$-convolution of tensor fields. It is known by specialists in the field that the two approaches are equivalent, with steerable convolution being the Fourier transform of $\mathrm{SE}(3)$ convolution. Unfortunately, these results are not widely known and moreover the exact relations between deep learning architectures built upon these two approaches have not been precisely described in the literature on equivariant deep learning. In this work we provide an in-depth analysis of both methods and their equivalence and relate the two constructions to multiview convolutional networks. Furthermore, we provide theoretical justifications of separability of $\mathrm{SE}(3)$ group convolution, which explain the applicability and success of some recent approaches. Finally, we express different methods using a single coherent formalism and provide explicit formulas that relate the kernels learned by different methods. In this way, our work helps to unify different previously-proposed techniques for achieving roto-translational equivariance, and helps to shed light on both the utility and precise differences between various alternatives. We also derive new TFN non-linearities from our equivalence principle and test them on practical benchmark datasets.

==> Harmonic_SE3_Convolution.tex <==
\section{Harmonic representation of $\mathrm{SO}(3)$ and $\mathrm{SE}(3)$ convolutions}

\label{sec:harmonic_representations}

\Adrien{Although proofs will be in the appendix we will probably need to provide some more intuition here}

Let $f: \mathrm{SE}(3) \rightarrow \RR$ be a smooth function. By  $\cref{th:so3_hilbert_basis}$, for all $x \in \RR^3$ the function $f(x, \bullet)$ admits a decomposition in the Wigner basis:
\begin{equation}
f(x, \bullet) = \sum_{\ell = 0}^{+\infty} \langle f^{\ell}(x), D^{\ell} \rangle
\label{eq:se3_fn_pt_decomposition}
\end{equation}
where for each $\ell \in \NN$, $f^{\ell}(x) \in \RR^{(2\ell+1)\times(2\ell+1)}$ is the matrix of coefficients of $f(x, \bullet)$ w.r.t. the Wigner matrix $D^{\ell}$. 

\begin{Theorem}
The the Wigner coefficients of the convolution between two smooth functions $f,g: \mathrm{SO}(3) \rightarrow \RR$ are given by:
\[
(f \ast_{\mathrm{SO}(3)} g)^{\ell} = f^{\ell} g^{\ell}.
\]
\end{Theorem}
\iffalse
\begin{proof}
\[
\begin{aligned}
&
f \ast_{\mathrm{SO}(3)} g(R) 
\\
&
= 
\int \sum_{\ell} \langle f^{\ell}, D^{\ell}(H) \rangle \sum_{\ell'} \langle g^{\ell'}, D^{\ell'}(H^{-1}R) \rangle dH
=
\int \sum_{\ell} \langle f^{\ell}, D^{\ell}(H) \rangle \sum_{\ell'} \langle g^{\ell'}, D^{\ell'}(H)^{\top}D^{\ell'}(R) \rangle dH
\\
&
=
\int \sum_{\ell} \langle f^{\ell}, D^{\ell}(H) \rangle \sum_{\ell'} \langle D^{\ell'}(R)(g^{\ell'})^{\top},  D^{\ell'}(H) \rangle dH
=
 \sum_{\ell\ell'} \int \langle f^{\ell} \otimes D^{\ell'}(R)(g^{\ell'})^{\top}, D^{\ell}(H) \otimes D^{\ell'}(H) \rangle \rangle dH
 \\
 &
 =
 \sum_{\ell} \int \langle f^{\ell} \otimes D^{\ell}(R)(g^{\ell})^{\top}, D^{\ell}(H) \otimes D^{\ell}(H) \rangle \rangle dH
 =
 \sum_{\ell} \sum_{ij} f^{\ell}_{ij} (D^{\ell}(R) (g^{\ell})^{\top})_{ij}
\\
&
=
\sum_{\ell} \langle f^{\ell}, D^{\ell}(R) (g^{\ell})^{\top} \rangle
=
\sum_{\ell} \langle f^{\ell}g^{\ell} , D^{\ell}(R) \rangle
\end{aligned}
\]
\end{proof}
\fi

\begin{Lemma}[Wigner decomposition of separable $\mathrm{SE}(3)$ convolution]
Let $f: \mathrm{SE}(3) \rightarrow \RR$ be a smooth function. The Wigner coefficients at $x \in \RR^3$ of the convolutions $g := f \ast (\kappa^{\ell'}_{nm} \otimes \delta_I)$ between $f$ and a steerable kernel basis $\kappa^{\ell'}_n$ over $\RR^3$ are given by:
\[
\begin{aligned}
&
(f \ast (\kappa^{\ell'}_{nm} \otimes \delta_I))^L_{ij}
=
\sum_{\ell}  Q^{L, (\ell, \ell')}_{i,:,:}  \left(f^{\ell} \ast_{\RR^3} \kappa^{\ell'}_{n}\right) Q_{:,m,j}^{ (\ell, \ell'), L}
\\
&
(f \ast (\delta_0 \otimes \theta))^{L} =  f^{L}(x)\theta^{L}
\end{aligned}
\]
where the sum ranges over indices $\ell$ such that $|\ell - \ell'| \leqslant L \leqslant \ell + \ell'$.
\end{Lemma}

\begin{Theorem}[Harmonic decomposition of $\mathrm{SE}(3)$-convolution]
\label{th:harmonic_decomposition_se3_conv}
The Wigner coefficients of the $\mathrm{SE}(3)$-convolution layer introduced in 
\cref{th:conv_approx} are given by:
\[
\begin{aligned}
\mathrm{Conv}_{\mathrm{SE}(3)}(f, W)^L_{ij,d}
=
\sum_{\ell\ell'cnk}
 Q^{L, (\ell, \ell')}_{i,:,:}  \left(f^{\ell}_{:,k,c} \ast_{\RR^3} \kappa^{\ell'}_{n}\right) 
 \sum_{mk'} Q_{k,m,k'}^{ (\ell, \ell'), L} W^{\ell', L}_{cnmk',jd}
\end{aligned}
\]
\end{Theorem}

\iffalse
\begin{Theorem}[Wigner decomposition of separable $\mathrm{SE}(3)$ convolution]
Let $f: \mathrm{SE}(3) \rightarrow \RR$ be a smooth function. The Wigner coefficients at $x \in \RR^3$ of the convolutions $g := f \ast (\kappa^{\ell'}_{nm} \otimes \delta_I)$ between $f$ and a steerable kernel basis $\kappa^{\ell'}_n$ over $\RR^3$ are given by:
\[
g^L(x) = \sum_{\ell=a(L,\ell')}^{b(L,\ell')}  Q^{L, (\ell, \ell')}  \left(f^{\ell} \ast_{\RR^3} \kappa^{\ell'}_{n}(x)\right) \left(I_{2\ell+1} \otimes (\delta_m^{\ell'})^{\top}\right) Q^{ (\ell, \ell'), L}
\]
where $a(L, \ell') := \max(L-\ell',0)$, $b(L, \ell') := \mathbb{1}_{\ell' \leqslant \ell}(L+\ell') + \mathbb{1}_{\ell' < \ell}(\ell'-L)$ and $\delta^{\ell'}_m \in \RR^{2\ell'+1}$ is the vector defined by $(\delta^{\ell'}_m)_{i} := \delta_{im}$. We have:
\[
f \ast (\kappa^{\ell'}_{nm} \otimes \delta_I)(x,R) = \sum_{L=0}^{+\infty} \langle g^L(x), D^L(R) \rangle. 
\]
The Wigner coefficients at $x \in \RR^3$ of the convolution $h := f \ast (\delta_0 \otimes \theta)$ between $f$ and a function $\theta: \mathrm{SO}(3) \rightarrow \RR$ are given by:
$
h^{\ell} = f^{\ell}(x) \theta^{\ell}
$ 
i.e. 
\[
f \ast (\delta_0 \otimes \theta)(x,R) = \sum_{\ell=0}^{+\infty} \langle f^{\ell}(x)\theta^{\ell}, D^{\ell}(R) \rangle.
\]
where $(\theta^{\ell})_{\ell}$ are the coefficients of $\theta$ in the Wigner basis.
\end{Theorem}
\begin{proof}
We have:
\[
\begin{aligned}
f \ast (\kappa^{\ell'}_{nm} \otimes \delta_I) (x, R)
&
=
\int_{\RR^3} f(t,R) \kappa^{\ell'}_{nm}(R^{-1}(x-t))\mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty} \int_{\RR^3} \langle f^{\ell}(t), D^{\ell}(R) \rangle \sum_{m'=-\ell'}^{\ell'}D^{\ell'}(R)^{\top}_{mm'} \kappa^{\ell'}_{nm'}(x-t)\mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty} \int_{\RR^3} \langle f^{\ell}(t), D^{\ell}(R) \rangle  \langle D^{\ell'}(R)^{\top} \kappa^{\ell'}_{n}(x-t), \delta_m^{\ell'} \rangle \mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty} \int_{\RR^3} \langle f^{\ell}(t), D^{\ell}(R) \rangle  \langle D^{\ell'}(R)^{\top} , \delta_m^{\ell'} \kappa^{\ell'}_{n}(x-t)^{\top} \rangle \mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty} \int_{\RR^3} \langle f^{\ell}(t), D^{\ell}(R) \rangle  \langle \kappa^{\ell'}_{n}(x-t)(\delta_m^{\ell'})^{\top}, D^{\ell'}(R)  \rangle \mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty} \int_{\RR^3} \langle f^{\ell}(t) \otimes \kappa^{\ell'}_{n}(x-t)(\delta_m^{\ell'})^{\top}, D^{\ell}(R) \otimes D^{\ell'}(R) \rangle \mathrm{d}t
\\
&
=
\sum_{\ell=0}^{+\infty}  \sum_{L=|\ell - \ell'|}^{\ell+\ell'}\int_{\RR^3} \langle f^{\ell}(t) \otimes \kappa^{\ell'}_{n}(x-t)(\delta_m^{\ell'})^{\top}, Q^{(\ell, \ell'),L}D^L(R)Q^{L, (\ell, \ell')}  \rangle \mathrm{d}t
\\
&
=
\sum_{L=0}^{+\infty} \sum_{\ell=a(L, \ell')}^{b(L, \ell')}\int_{\RR^3} \langle Q^{L, (\ell, \ell')} f^{\ell}(t) \otimes \kappa^{\ell'}_{n}(x-t)(\delta_m^{\ell'})^{\top} Q^{ (\ell, \ell'), L}, D^L(R)  \rangle \mathrm{d}t
\\
&
=
\sum_{L=0}^{+\infty}  \langle \sum_{\ell=a(L, \ell')}^{b(L, \ell')} \langle Q^{L, (\ell, \ell')} \int_{\RR^3} f^{\ell}(t) \otimes \kappa^{\ell'}_{n}(\delta_m^{\ell'})^{\top}(x-t) \mathrm{d}t \  Q^{ (\ell, \ell'), L}, D^L(R)  \rangle 
\\
&
=
\sum_{L=0}^{+\infty}   \langle \sum_{\ell=a(L, \ell')}^{b(L, \ell')}  \langle Q^{L, (\ell, \ell')}  \left(f^{\ell} \ast_{\RR^3} \kappa^{\ell'}_{n}(x)\right) \left(I_{2\ell+1} \otimes (\delta_m^{\ell'})^{\top}\right) Q^{ (\ell, \ell'), L}, D^L(R)  \rangle
\end{aligned}
\]
\end{proof}
\fi

==> Harmonic_bases.tex <==
\section{Harmonic and steerable kernel bases}

\Adrien{This can be heavily cut down, many details can be sent to the appendix, we need good references for the results we do not directly prove}
\label{sec:harmonics}



In this section we recall the basic definition and properties of harmonic bases that we use throughout this work. We provide explicit formulas and additional details in the appendix. 

\subsection{Spherical harmonics \& Wigner matrices}

Spherical harmonics are homogeneous polynomial functions, over $\RR^3$, for each $\ell \in \NN^*$ there are $2\ell + 1$ degree $\ell$ spherical harmonics denoted $Y_{\ell,-\ell}, \dots, Y_{\ell,\ell}$ a key property of spherical harmonics fundamental to many equivariant neural networks designs \Adrien{cite} is their rotation equivariance:

\begin{Theorem}[Rotation of Spherical Harmonics]
For all $x \in \RR$
let $Y_{\ell}(x) := (Y_{\ell,-\ell}, \dots, Y_{\ell,\ell})$ be the vector of degree $\ell$ spherical harmonics at $x$. Then for all $R \in \mathrm{SO}(3)$ there exist a matrix $D^{\ell}(R) \in \mathrm{SO}(2\ell+1)$ called the (degree $\ell$) Wigner matrix, such that:
\[
Y_{\ell}(Rx) = D^{\ell}(R)Y_{\ell}(x).
\]
\end{Theorem}

The Wigner matrices are the so called \textbf{irreducible representation} of $\mathrm{SO}(3)$ by  Peter-Weyl theorem \Adrien{ref} the coefficients of these matrices form a Hilbert basis of the space $L^{2}(\mathrm{SO}(3))$ of square integrable functions over $\mathrm{SO}(3)$ for its Haar measure:

\begin{Theorem}[The Wigner Basis]
The Wigner matrices coefficients form a Hilbert basis of $L^{2}(\mathrm{SO}(3))$, that is:
\begin{enumerate}
    \item For all $\ell,m,n$ and $\ell',m',n'$ such that the coefficients $D^{\ell}_{mn}$ and $D^{\ell'}_{m'n'}$ are defined we have:
\[
\int_{R} \hspace{-1mm} (D_{mn}^{\ell}D_{m'n'}^{\ell'})(R) \mathrm{d}R
=
\delta_{\ell\ell'}\delta_{mm'}\delta_{nn'}.
\]
\item For any square integrable function $f:\mathrm{SO}(3) \rightarrow \RR$ uniquely decomposes in the Wigner basis, i.e. for all $R \in \mathrm{SO}(3)$:
$
f(R) = \sum_{\ell \geqslant 0} \langle f^{\ell}, D^{\ell}(R)\rangle
$
where for each $\ell \in \NN$, $f^{\ell} \in \RR^{(2\ell+1, 2\ell+1)}$ is the matrix of coefficients of $f$ associated with $D^{\ell}$.
\item Furthermore the coefficient matrices of $f$ satisfy the equivariance relation $(R.f)^{\ell} = D^{\ell}(R)f^{\ell}$ for all $\ell \in \NN, R\in \mathrm{SO}(3)$, where $(R.f)(x) := f(R^{-1}x)$. 

\end{enumerate}
\label{th:so3_hilbert_basis}
\end{Theorem}

Convolution features computed with
3D Convolution kernels based on spherical harmonics (also called steerable kernels) inherit their rotation equivariance properties forming the foundational bloc of many equiavriant designs \Adrien{CITE}.

\begin{Definition}[3D steerable kernel basis]
A $3D$ steerable kernel basis $\kappa$ is a finite dimensional basis of functions $\kappa_{rm}^{\ell}: \RR^3 \rightarrow \RR$ of the form:
\[
\kappa_{rm}^{\ell}(x) := \varphi_{r}^{\ell}(\Vert x \Vert_2^2) Y^{\ell}_m(x), \ \ \forall x \in \RR^3.
\]
where $\varphi_{r}^{\ell}: \RR \rightarrow \RR$ is the radial component, and the angular component is given by spherical harmonics. 
\end{Definition}
A typical choice for the radial component $\varphi_r$ is normalized Gaussian shell functions of the form:
$
\varphi_r(t) := \frac{1}{t^{\ell / 2}} \exp \left( \frac{(\sqrt{t} - \rho_r^{\ell})^2}{2(\sigma_r^{\ell})^2}\right)
$
where $\rho_r^{\ell}$ is the radius of the shall and the standard deviation parameter $\sigma_r^{\ell}$ controls its width. The $\frac{1}{t^{\ell / 2}}$ factor is normalizing the spherical harmonic component, as spherical harmonics are homogeneous polynomials we can normalize the input to the spherical harmonics instead. We discuss other choices of radial functions in the appendix \Adrien{ref zernike}


\subsubsection{Decomposing products of spherical harmonics \& Wigner matrices}

\begin{Definition}[Clebsch-Gordan coefficients]
The Clebsch-Gordan coefficients are defined for any $\ell,\ell' \in \NN$, $m \in \llbracket -\ell, \ell \rrbracket, m' \in \llbracket -\ell, \ell \rrbracket$ and $L \in \llbracket |\ell-\ell'|, \ell+\ell' \rrbracket$ such that $\ell \geqslant \ell'$ and $M \in \NN$ by:
\[
\begin{aligned}
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle 
\\
:= \ 
&\delta_{M,m+m'} \sqrt{\frac{(2L+1)(L+\ell-\ell')!(L-\ell+\ell')!(\ell+\ell'-L)!}{(\ell+\ell'+L+1)!}}\ \times \\
&\sqrt{(L+M)!(L-M)!(\ell-m)!(\ell+m)!(\ell'-m')!(\ell'+m')!}\ \times \\
&\sum_k \frac{(-1)^k}{k!(\ell+\ell'-L-k)!(\ell-m-k)!(\ell'+m'-k)!(L-\ell'+m+k)!(L-\ell-m'+k)!}.
\end{aligned}
\]
The definition extends to $M < 0$ and $\ell < \ell'$ using the relations:
\[
\begin{aligned}
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle := (-1)^{L-\ell-\ell'}\langle \ell,\ell';-m,-m'|\ell,\ell';L,-M\rangle
\\
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle := (-1)^{L-\ell-\ell'} \langle \ell',\ell;m',m|\ell',\ell;L,M\rangle
\end{aligned}
\]
For convenience we define the sparse tensors $Q^{L, (\ell,\ell')} \in \RR^{(2L+1)\times (2\ell+1) \times (2\ell'+1)}$ and its transpose \newline $Q^{(\ell,\ell'),L} \in \RR^{(2\ell+1) \times (2\ell'+1) \times (2L+1)}$ by:
\[
Q^{(\ell,\ell'), L} := (C^{\ell} \otimes C^{\ell'}) \Tilde{Q}^{(\ell,\ell'), L} (C^{\ell})^*, \ \
Q^{L, (\ell,\ell')} :=  C^{\ell} \Tilde{Q}^{L, (\ell,\ell')}  ((C^{\ell})^* \otimes (C^{\ell'})^*)
\]
Where the tensors $\Tilde{Q}^{L, (\ell,\ell')}$ and $\Tilde{Q}^{L, (\ell,\ell'), L}$ are sparse tensors whose non zero coefficients are given by the Clebsch-Gordan coefficients:
\[
\Tilde{Q}^{(\ell,\ell'), L}_{m, m', m+m'} := \Tilde{Q}^{L, (\ell,\ell')}_{m+m', m, m'} := \langle \ell,\ell'; m,m' | \ell,\ell'; L, \left(m + m'\right) \rangle.
\]


\iffalse
\[
Q^{L, (\ell,\ell')}_{m+m'+L, (2\ell'+1)(m+\ell) + m'+\ell'} = \langle \ell,\ell'; m,m' | \ell,\ell'; L, \left(m + m'\right) \rangle.
\]
\fi
\end{Definition}

\begin{Theorem}[Orthogonality relation of Clebsch-Gordan coefficients]
For any $\ell, \ell' \in \NN$ and $L \in \llbracket |\ell - \ell'|, \ell + \ell' \rrbracket$ we have:
\[
\sum_{L = |\ell-\ell'|}^{\ell+\ell'} Q^{(\ell, \ell'), L} Q^{L, (\ell, \ell')} = I_{(2\ell+1)(2\ell'+1)}, \ \ Q^{L, (\ell, \ell')} Q^{(\ell, \ell'),L'} = \delta_{L,L'} I_{2L+1}
\]
\end{Theorem}

\begin{Theorem}[Decomposition of spherical harmonics \& Wigner products]
\label{th:clebsh_gordan_decomposition}
For any $\ell, \ell' \in \NN$ and $L \in \llbracket |\ell - \ell'|, \ell + \ell' \rrbracket$ we have:
\[
\begin{aligned}
&
Y^{\ell} \otimes Y^{\ell'} = \sum_{L=|\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}Y^L, \ \ \ Y^L = Q^{L,(\ell, \ell')} (Y^{\ell} \otimes Y^{\ell'})
\\
&
D^{\ell} \otimes D^{\ell'} = \sum_{L=|\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}D^LQ^{L, (\ell, \ell')}, \ \ \ D^L = Q^{L,(\ell, \ell')} (D^{\ell} \otimes D^{\ell'}) Q^{(\ell, \ell'), L}.
\end{aligned}
\]
\iffalse
\[
Y^{\ell}_m Y^{\ell'}_{m'} = \sum_{L = |\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}_{M,m,m'} Y^{L}_M
\]
\fi
\end{Theorem}

\iffalse
 In this work we consider steerable kernels given by the Zernike basis (defined below) which also forms a Hilbert basis of the Hilbert space $L^{2}(\mathcal{B}_3)$ of square integrable functions on the unit ball $\mathcal{B}_3 \subset \RR^3$.

\begin{Definition}[Zernike polynomials (radial)]
For all $\ell, n \in \NN$ such that $n - \ell \geqslant 0$ and $2 | (n - \ell)$ the (radial) Zernike polynomial $R_{n}^{\ell}$ is a degree $k = (n - \ell) / 2$ polynomial function on the real line defined for all $x \in \RR$ by:
\[
R_{n}^{\ell}(x) = \sum_{v=0}^k R_{n,v}^{\ell} x^v
\]
whose coefficient $R_{n,v}^{\ell}$ is given by:
\[
R_{n,v}^{\ell} :=
\frac{(-1)^k}{2^{2k}} \sqrt{\frac{2\ell + 4k + 3}{3}} \begin{pmatrix}
2k \\
k
\end{pmatrix}
(-1)^v
\frac{
\begin{pmatrix}
k \\
v
\end{pmatrix}
\begin{pmatrix}
2(k+\ell+v)+1 \\
2k
\end{pmatrix}}{\begin{pmatrix}
k+\ell+v \\
k
\end{pmatrix}}.
\]
\end{Definition}

\begin{Theorem}[Orthogonality of (radial) Zernike polynomials]
For all $\ell \in \NN$ the type $\ell$ (radial) Zernike polynomials form an orthogonal family for the push forward of Lebesgue's volume measure on the unit ball to the unit interval $[0, 1[$ by the norm function. More precisely, for all $\ell \in \NN$ and all $n,n'\in \NN$ such that $n,n' \geqslant \ell$ and $2|(n-\ell)$, $2|(n'-\ell)$ we have:
\[
\int_{r=0}^1 R_n^{\ell}(r)R_{n'}^{\ell}(r) r^2 \mathrm{d}r = 
\delta_{n,n'}.
\]
\end{Theorem}

\begin{Definition}[3D Zernike polynomials]
For any $\ell,n,m$ such that $n - \ell \geqslant 0$, $2|(n-\ell)$ and $m \in \llbracket -\ell, \ell \rrbracket$ the 3D Zernike polynomial $Z^{\ell}_{nm}$ is a degree $n$ polynomial functions over $\RR^3$ defined for all $(x,y,z) \in \RR^3$ by:
\[
Z^{\ell}_{nm}(x,y,z) := R_n^{\ell}(x^2 + y^2 + z^2)Y_m^{\ell}(x,y,z).
\]
\end{Definition}

\begin{Theorem}[Hilbert basis of $L^2(\mathcal{B}_3)$]
The 3D Zernike polynomials, form a Hilbert basis of the Hilbert space $L^2(\mathcal{B}_3)$ of square integrable functions on the unit ball $\mathcal{B}_3 \subset \RR^3$, that is, for any $n,\ell,m$ and $n',\ell',m'$ such that the Zernike polynomials $Z_{nm}^{\ell}$ and $Z_{n'm'}^{\ell'}$ are defined we have:
\[
\frac{3}{4\pi}\int_{x \in \mathcal{B}_3} Z_{nm}^{\ell}(x)Z_{n'm'}^{\ell'}(x) \mathrm{d}x
=
\delta_{nn'} \delta_{\ell\ell'} \delta_{mm'}.
\]
\end{Theorem}
\fi

==> Relation_To_General_Theory.tex <==
\section{Relation to the general Theory of Cohen \textit{et al}}

In this section we describe at a very high level the relation between this work and the general theory of
equivariant neural networks presented in \cite{kondor2018generalization, cohen2018intertwiners, cohen2019general, esteves2020theoretical, lang2020wigner} more specifically the decomposition of $\mathrm{SE}(3)$ convolution in the Wigner basis presented in \cref{th:tfn_vs_se3_conv_1} can be recovered from the theory of Cohen \textit{et al} \cite{cohen2019general} and the expression of 3D steerable CNNs \cite{weiler20183d}. We believe the added value of our work is to state this result explicitly in terms of $\mathrm{SE}(3)$-convolution and to establish an explicit equivalence between TFN and $\mathrm{SE}(3)$ convolution layers in \cref{th:tfn_vs_se3_conv_2}, we hope our presentation highlight these results and will make them more accessible. We now describe how the expression of $\mathrm{SE}(3)$ convolution from our $\cref{th:tfn_vs_se3_conv_1}$ follows from \cite{weiler20183d, cohen2019general}. At a very high level \cite{weiler20183d} introduces the notion of 3D steerable CNNs, starting from classical 3D convolution and establishing necessary and sufficient condition on the kernel bases to achieve equivariance. This construction is further generalized in \cite{cohen2019general}, given a locally compact unimodular group $G$ \cite{cohen2019general} shows that any equivariant linear functional map mapping functions on $G$ to functions on $G$ can be realized a $G$-convolution by a kernel $\kappa:G \rightarrow \RR$ and shows different ways of representing the kernel $G$ under different assumptions on the group structure of $G$. In particular assuming $G$ has a compact normal subgroup $H$. 




using the language of fiber bundles and group representations. 

A representation of a group $H$ is a linear action of $H$ onto a vector space, the typical representation of a group $H$ is the action of $H$ on functions defined over $H$ given by $(g.f)(x) := f(g^{-1}x)$ for any $f:H \rightarrow \RR$ and $g,x \in H$. When $H$ is compact we can find a suitable function basis in which this action is bloc diagonal with blocs of minimal size, this result is known as the Peter Weyl theorem (see Esteves survey \cite{esteves2020theoretical} and \Adrien{add a specialized ref}).  \cref{th:so3_hilbert_basis} is the case where $H = \mathrm{SO}(3)$, the Wigner basis bloc-diagonalizes rotation of functions, the action on their Wigner coefficients is given by the Wigner matrices as stated in 3). 

A key result from \cite{cohen2019general} is that Given a group $G$ and a compact subgroup $H \subseteq G$

A fiber bundle is a space that locally looks like a product space it consist of a projection $\mathrm{pr}: E \rightarrow B$ from a total space $E$ to a base space $B$ such that 




a general construction for $\mathrm{}$




Cohen \textit{et al} \cite{cohen2019general}. More specifically we explain how our results on the decomposition of $\mathrm{SE}(3)$-convolution in the Wigner basis \cref{th:tfn_vs_se3_conv_1} and the equivalence between $\mathrm{SE}(3)$-convolution layers and TFN layers \cref{th:tfn_vs_se3_conv_2} follow from the theory. \Adrien{we must explain what is the added value, I think this should be done in the abstract / intro / related work essentially we provide an explicit statment of the result in the case of $\mathrm{SE}(3)$-convolution and we start from $\mathrm{SE}(3)$ convolution itself rather than going through the theory of steerable kernels and its relation to group convolution, we can say just that in the intro + say this more user / reader friendly making this result more accessible, and develop here}.

\Adrien{Insert high level description of the theory here, this can be short and take a couple paragraphs, representations \& steerable kernels + relation to $\mathrm{SE}(3)$-conv}.

==> SE3_Convolution.tex <==
\subsection{$\mathrm{SO}(3)$ and $\mathrm{SE}(3)$ convolution}
\label{sec:se3_conv}



\subsubsection{Continuous $\mathrm{SE}(3)$-convolution}



The general definitions from \cref{sec:g_conv} specialize to the roto-translation group $\mathrm{SE}(3)$ for, which we recall the definition below before defining $\mathrm{SE}(3)$-convolution.

\begin{Definition}[The roto-translation group $\mathrm{SE}(3)$]
the roto-translation group $\mathrm{SE}(3) = \RR^3 \rtimes \mathrm{SO}(3)$ is the semi direct product between the translation group $\RR^3$ and the rotation group $\mathrm{SO}(3)$ and that it's composition law is given by:
$
(x, U).(y, V) = (Uy + x, UV), \ \ (t, H)^{-1} := (H^{-1}, -H^{-1}t)
$.
\end{Definition}

A key component to the construction of group convolution is the underlying measure $\nu$, a canonical choice consists of a product of Haar measures on $\RR^3$ and $\mathrm{SO}(3)$, more specifically the canonical Haar measure of $\mathrm{SE}(3)$ is $\nu = \lambda \otimes \mu$ where $\lambda$ is the Lebesgues measure on $\RR^3$ and $\mu$ is the volume measure of $\mathrm{SO}(3)$ we refer to the appendix \Adrien{add some ref} for more details on $\mu$.




\iffalse
which we now describe in the coordinate system given by Euler angles parametrization of $\mathrm{SO}(3)$. For any $\theta \in \RR$ $R_X(\theta), R_Y(\theta), R_Z(\theta) \in \mathrm{SO}(3)$ the rotations of angle $\theta$ around the $x, y$ and $z$ axes respectively.
\begin{Theorem}[Euler angle parametrization of $\mathrm{SO}(3)$]
The Euler angles map 

\[
\begin{array}{rcl}
R_{ZYZ} : [0, 2\pi] \times [0, \pi] \times [0, 2\pi] &\longrightarrow \mathrm{SO}(3) \\
     (\alpha, \beta, \gamma) &\longmapsto R_{Z}(\alpha)R_{Y}(\beta)R_{Z}(\gamma) 
\end{array}
\]
is a surjection whose restriction to $[0, 2\pi[ \times [0, \pi[ \times [0, 2\pi[$ is injective and its image is a dense open subset of $\mathrm{SO}(3)$.
\end{Theorem}

\begin{Theorem}[Haar Measure of $\mathrm{SO}(3)$]
The riemannian metric of $\mathrm{SO}(3)$ is the the metric induced by the inclusion $\mathrm{SO}(3) \hookrightarrow \mathrm{M}_{3,3}(\RR) \simeq \RR^9$. The Haar measure $\mu$ of $\mathrm{SO}(3)$ is the measure induced by its riemannian metric. The pull back of the volume form $\omega$ associated with the riemannian metric of $\mathrm{SO}(3)$ by the Euler angles map $R$ has the following expression in the canonical coordinate system $(\alpha, \beta, \gamma)$ of $[0, 2\pi[ \times [0, \pi[ \times [0, 2\pi[$:
\[
R_{ZYZ}^*\omega = \sin(\beta) d\alpha \wedge d\beta \wedge d\gamma.
\]
that is, parametrizing $\mathrm{SO}(3)$ by $[0, 2\pi[ \times [0, \pi[ \times [0, 2\pi[$ the density of $\mu$ w.r.t. the Lebesgues measure $\lambda$ is given by $\frac{d\mu}{d\lambda}(\alpha, \beta, \gamma) = \sin(\beta)$.
\end{Theorem}
\fi 


Following the general definition of group convolution (\cref{def:g_conv}) we obtain the definition of $\mathrm{SE}(3)$-convolution:

\begin{Definition}[$\mathrm{SE}(3)$-convolution]
\label{def:se3_conv}
$\mathrm{SE}(3)$-convolution is defined for any $f,g: \mathrm{SE}(3) \rightarrow \RR$ by:
\begin{equation}
(f  \ast g) (x, R) :=
\int_{\RR^3}  \int_{\mathrm{SO}(3)} f(t,H)g(H^{-1}(x-t), H^{-1}R) d\mu(H) d\lambda(t)
\label{eq:se3_conv}
\end{equation}
\end{Definition}


Note that $\mathrm{SE}(3)$-conv layers operate over functions on $\mathrm{SE}(3)$ and so do $\mathrm{SE}(3)$-CNNs. We are interested in networks which operate over functions on $\RR^3$ and are equivariant to rotation of this input. A simple way to adapt $\RR^3$ inputs to $\mathrm{SE}(3)$-CNNs is to do straightforward extension to $\mathrm{SE}(3)$, that is, any function $f:\RR^3 \rightarrow \RR$ naturally extends to a function $\Tilde{f}: (x, R) \in \mathrm{SE}(3) \mapsto f(x)$.

\subsubsection{$\mathrm{SE}(3)$-convolution on point clouds}

In practice we are interested in networks that operate on pointclouds as continuous networks are not suitable for practical implementation \Adrien{At least not directly}, first we observe that \cref{def:pointcloud_convolution} of point cloud convolution can be reformulated within our formalism of \cref{sec:g_conv}. We consider  $\RR^3$-convolution i.e. group convolution from \cref{def:g_conv} with $G = \RR^3$ and setting the measure to be the sum of Dirac measures $\delta_X := \sum_i \delta_{X_i}$ over a pointcloud $X$. We note that the resulting function $f \ast_{\delta_X} \kappa$ is defined on the hole of $\RR^3$ instead of just the pointcloud $X$ but its restriction to $X$ coincides with pointcloud convolution from \cref{def:pointcloud_convolution} and the convolution $f \ast_{\delta_X} \kappa$ depends only on the values of $f$ over $X$ therefore a CNN $\mathrm{CNN}_{\RR^3, \delta_X}$ as defined in \cref{def:gcnn} would coincide with pointcloud CNNs using pointcloud convolutions \cref{def:pointcloud_convolution}. We extend this idea to $\mathrm{SE}(3)$ convolution by setting $\lambda = \delta_X$ in \cref{def:se3_conv}, (i.e. $\nu = \delta_X \otimes \mu)$. We note that with our definition $\mu$, the $\mathrm{SO}(3)$ component of the measure is still continuous we will show how it can be discretized \Adrien{ref corresponding section}. All in all, we can use $\lambda$ to be Lebesgue's measure on $\RR^3$ or $\lambda = \delta_X$ indiscriminately in our analysis avoiding parallel discussions of the discrete and continuous case. \Adrien{should we say $h.\delta_X = \delta_{h.X}$ for $h \in \mathrm{SE}(3)$ ?}. 





\iffalse
\paragraph{Note} In \cref{def:se3_conv}
of $\mathrm{SE}(3)$-convolution we assumed $\lambda$ is the Lebesgue's measure of $\RR^3$, in practice this is discredtized using the notion of pointcloud convolution which can be defined by replacing  $\lambda$ by a finite sum of Dirac measures over points of $\RR^3$. This alternative assumption does not affect the general discussion and all results presented in this work also hold in this setting. 


\begin{Definition}[Point-cloud based $\mathrm{SE}(3)$-CNNs]
\label{def:pc_se3_cnns}
A $\mathrm{SE}(3)$-CNN over a pointcloud $X$ is a special case of $\mathrm{SE}(3)$-CNN based on the measure $\nu = \delta_X \otimes \mu$ with $\delta_X := \sum_i \delta_{X_i}$ and taking functions supported by $X \times \mathrm{SO}(3)$ as input.
\end{Definition}

 
\paragraph{Note} In \cref{def:pc_se3_cnns} we chose to only discretize the $\RR^3$ component of the convolutions. Previous works \Adrien{(CITE)} consider a discretization of the $\mathrm{SO}(3)$ component as well restricting the convolution to a finite subgroup of $\mathrm{SO}(3)$ like the isocahedral group. In \cref{sec:harmonic_representations} we describe harmonic decomposition of $\mathrm{SE}(3)$-convolution which offers an other way of discretizing the $\mathrm{SO}(3)$ component.
\fi











==> Standard_Convolution.tex <==
\subsection{Euclidean and Pointcloud Convolution}
\label{sec:euclidean_pc_conv}

Convolution is the cornerstone of Convolutional Neural Networks for image analysis popularized by the famous AlexNet \cite{krizhevsky2012imagenet}. In this section we recall the classical definition of Euclidean convolution and its counterpart for discrete pointclouds. 

%\Adrien{discussion on domains added here}
In the continuous setting, standard Euclidean convolution is defined between a function $f$ and a kernel $\kappa$, where both $f, \kappa: \RR^d \rightarrow \RR$, and is defined as:
\begin{equation}
	f \ast \kappa(x) := \int_{\RR^d} f(t)\kappa(x-t)dt
	\label{eq:euclidean_conv}
\end{equation}
Note that in practice \textit{cross-correlation} is often preferred over convolution. Cross-correlationcan be obtained from convolution by negating the input of the kernel, replacing $\kappa$ by $:x \mapsto \kappa(-x)$ in \cref{eq:euclidean_conv}. In this work we refer to both as convolution as our analysis applies to both notions. 


The definition of convolution, can be adapted to the case of discrete point clouds, where we assume that the input signal is only defined on the given set of points $X$, i.e., $f: X \rightarrow \RR$, while $\kappa$ is a learnable kernel over $\RR^3 \rightarrow \RR$. This leads to:
\begin{Definition}[Pointcloud Convolution]
	\label{def:pointcloud_convolution}
	Given a point cloud $X \in \RR^{(N,3)}$ seen as a subset of $\RR^3$ the convolution of a function $f:X \rightarrow \RR$ by a kernel $\kappa: \RR^3 \rightarrow \RR$ is the function over $X$ defined by:
	\[
	f \ast_X \kappa( X_i ) := 
	\sum_{j} f(X_j)\kappa(X_i - X_j).
	\]
\end{Definition}

Multiple works investigate the idea of convolution for point clouds \cite{atzmon2018point, hermosilla2018monte, hua2018pointwise, li2018pointcnn, xu2018spidercnn, thomas2019kpconv} these works propose variations of \cref{def:pointcloud_convolution} given above. The main variations consist in developing methods to compensate biases induced by uneven non uniform or uneven sampling, some works like \cite{atzmon2018point} normalize the signals, others use Monte Carlo integration with re-sampling \cite{hermosilla2018monte} and others learn the kernel functions themselves in addition to the weights \cite{thomas2019kpconv}.


  



% of pointcloud convolution discretizing the continuous case from \cref{eq:euclidean_conv}:

%In the case of point clouds, convolution is defined between a signal on a point cloud and a kernel over $\RR^3$ in both cases the signal is compared to the kernel via L2 product across all translations of the kernel, this gives a signal over $\RR^3$ (or the point-cloud) representing the correlation between the signal and the kernel in a given pose at every space (or point-cloud) locations. 


\iffalse
In this work we are also interested in correlations between the kernel and the signal across different poses. This naturally leads to signals (resp. kernels) defined on the group $\mathrm{SE}(3) := \RR^3 \rtimes \mathrm{SO}(3)$ of translations and rotations \Adrien{to model responses over different poses (resp. correlate/aggregate information across poses)}

. This introduces the need to operate on functions over other domains. In \cref{sec:g_conv} we describe general group convolution between functions defined on a group and specialize it to $\mathrm{SO}(3)$ and $\SE(3)$ in \cref{sec:se3_conv}. \maks{Can we either give some references to papers that actually do this -- i.e., operate with signals defined over $\SE(3)$ or forward reference the discussion. Something like ``we mention several variants of this general idea used in practice, in Section X''} 
\fi







%The convolution of any two square integrable functions \Adrien{we can have other more restrictive assumptions eg: smooth compactly supported or tempered, at least these properties are stable by convolution} $f,\kappa: \RR^d \rightarrow \RR$ is the function defined for all $x$ by:

%During the past decade deep learning has seen a wide adoption across many disciplines including 3D shapes analysis \Adrien{processing ?}. Motivated by the success of CNNs for image analysis a lot of research effort have been carried to replicate the convolution like structures \Adrien{layers ?} for 3D data, perhaps the most straightforward extension is to consider 3D CNNs operating on voxel data as proposed by \cite{maturana2015voxnet}, this however is generally considered inefficient due to the large amount of voxels required to accurately describe a shape compared to sparser representations like meshes or pointclouds. A great number of approaches to define convolution like operations on meshes \cite{masci2015geodesic, monti2017geometric, poulenard2018multi, wiersma2020cnns} or pointclouds \cite{qi2017pointnet++, wang2019dynamic, atzmon2018point, li2018pointcnn, thomas2019kpconv} often broadening the notion of convolution, introducing non linear aggregations. In the "purest" sense convolution consist of moving a kernel along the input signal extracting local features in the same way regardless of the position. 







==> checklist.tex <==
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Realisation of multi-view-CNNs as $\mathrm{SE}(3)$-CNNs is shown in \cref{th:multiview_cnn}. The equivalence between 3D Steerable Convolution and $\mathrm{SE}(3)$ convolution and the interpretation of 3D Steerable Convolution as Fourier transform of  $\mathrm{SE}(3)$ convolution are shown in \cref{th:tfn_vs_se3_conv_1} and \cref{th:tfn_vs_se3_conv_2}. Separability of $\mathrm{SE}(3)$-convolution is analysed in \cref{subsec:separability}}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations are discussed in the conclusion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We do not state the full set of assumption within the definitions and theorems statement themselves to avoid redundancies but we state at the beginning of \cref{sec:g_conv} the common hypotheses to all definitions and theorems}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are in the Appendix in Supplementary material}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNo{We ran a modified version of the TFN implementation of \cite{poulenard2021functional}, we only describe our modifications and refer to \cite{poulenard2021functional} for details}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{This data was not available for our baselines}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{our experiments are minimal and run on a single gpu}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We modified a code from \cite{poulenard2021functional} and mention it in \cref{sec:results}}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> harmonic_bases_old.tex <==
\section{Harmonic and steerable kernel bases}


\label{sec:harmonics}

\subsection{Spherical harmonics \& Wigner matrices}
\begin{Definition}[Spherical harmonics]
Spherical harmonics are homogeneous polynomial functions, over $\RR^3$, for each $\ell \in \NN^*$ there are $2\ell + 1$ degree $\ell$ spherical harmonics $Y_{-m}^{\ell}, \dots, Y_{m}^{\ell}$ defined for any $X = (x,y,z) \in \RR^3$ by:
\[
\begin{aligned}
&
Y_{-m}^{\ell}(x,y,z) := \sqrt{\frac{2\ell+1}{2\pi}} \overline{\Pi}^{\ell}_m(x, y, z)B_m(x,y), \ \ m > 0
\\
&
Y_0^{\ell}(x,y,z):= \sqrt{\frac{2\ell+1}{4\pi}} \overline{\Pi}^{\ell}_0(x, y, z)
\\
&
Y_m^{\ell}(x,y,z) := \sqrt{\frac{2\ell+1}{2\pi}} \overline{\Pi}^{\ell}_m(x, y, z)A_m(x,y), \ \ \ m > 0
\end{aligned}
\]
where:
\[
\begin{aligned}
&
A_m(x,y) := \sum_{p=0}^m x^m y^{m-p} \cos((m-p)\frac{\pi}{2}),
\ \ \ 
B_m(x,y) := \sum_{p=0}^m x^m y^{m-p} \sin((m-p)\frac{\pi}{2})
\\
&
\overline{\Pi}^{\ell}_m(x, y, z) := \sqrt{\frac{(\ell-m)!}{(\ell+m)!}} \sum_{k=0}^{\lfloor (\ell - m)/2 \rfloor} (-1)^k 2^{\ell} \begin{pmatrix} \ell \\ k \end{pmatrix}\begin{pmatrix} 2\ell - 2k \\ \ell \end{pmatrix} \frac{(\ell - 2k)!}{(\ell - 2k - m)!} \Vert X \Vert^{2k}_2 z^{\ell - 2k - m}
\end{aligned}
\]
\end{Definition}




\begin{Theorem}[Hilbert basis of $L^2(\mathcal{S}_2)$]
The restriction of spherical harmonics to the unit sphere $\mathcal{S}_2 \subset \RR^3$ form a Hilbert basis of the space $L^2(\mathrm{S}_2)$ of square integrable functions on $\mathcal{S}_2$ for the surface measure of $\mathcal{S}_2$ whose density in the spherical coordinates $(\theta, \varphi) \in [0, 2\pi[ \times [0, \pi[$ is $\sin(\theta)$, that is, for any $\ell,m,\ell',m'$ we have:
\[
\int_{\varphi=0}^{2\pi} \int_{\theta=0}^{\pi} (Y^{\ell}_mY^{\ell'}_{m'})(\cos(\varphi)\sin(\theta), \sin(\varphi)\sin(\theta), \cos(\theta)) \sin(\theta) \mathrm{d}\theta \mathrm{d}\varphi = \delta_{\ell,\ell'}\delta_{m,m'}.
\]
\end{Theorem}



\subsubsection{Rotation of spherical harmonics}

We have described the real spherical harmonics. Complex spherical harmonics are related to real spherical harmonics by transition matrices. The transition matrix $C^{\ell} \in \mathcal{M}_{2\ell+1}(\CC)$ from complex to real spherical degree $\ell$ spherical harmonics is given by:
\[
\begin{cases}
\displaystyle C^{\ell}_{m,m} = {-i \over \sqrt{2}} & \text{if}\ m<0\\
\displaystyle C^{\ell}_{m,m} = {(-1)^m \over \sqrt{2}} & \text{if}\ m>0\\
\displaystyle C^{\ell}_{m,-m} = {1 \over \sqrt{2}} & \text{if}\ m<0\\
\displaystyle C^{\ell}_{m,-m} = {i(-1)^m \over \sqrt{2}} & \text{if}\ m>0\\
\displaystyle C^{\ell}_{0,0} = 1 & \\
\displaystyle C^{\ell}_{j,k} = 0 & \text{otherwise}
\end{cases}
\]
the transition from real to complex harmonics is given by the transpose conjugate matrix $(C^{\ell})^*$. 

\begin{Definition}[Wigner Matrix]
Let $\ell \in \NN$, The Wigner $d^{\ell}$ matrix is defined for any angle $\beta$ by:
\[
\begin{array}{lcl}
d^{\ell}_{m'm}(\beta) &=& [(\ell+m')!(\ell-m')!(\ell+m)!(\ell-m)!]^{1/2}
\sum\limits_s \left[\frac{(-1)^{m'-m+s}}{(\ell+m-s)!s!(m'-m+s)!(\ell-m'-s)!} \right.\\
&&\left. \cdot \left(\cos\frac{\beta}{2}\right)^{2\ell+m-m'-2s}\left(\sin\frac{\beta}{2}\right)^{m'-m+2s} \right].
\end{array}
\]
for $m, m' \in [|-\ell, \ell|]$ where the sum over $s$ is over such values that the factorials are non-negative. The complex Wigner $\Tilde{D}^{\ell}$ is defined for any angles $\alpha, \beta, \gamma$ by:
\[
\Tilde{D}^{\ell}(\alpha, \beta, \gamma) := e^{-im'\alpha}d^{\ell}_{m'm}(\beta)e^{-im\gamma}, \ \ m, m' \in [|-\ell, \ell|].
\]
The real Wigner matrix $D^{\ell}$ is defined by:
\[
D^{\ell} := C^{\ell} D^{\ell} (C^{\ell})^*
\]
\end{Definition}

\iffalse
For any angle $\theta$ we denote by $R_{X}(\theta), R_{Y}(\theta), R_{Z}(\theta) \in \mathrm{SO}(3, \RR)$ the rotations matrices around axis $x, y, z$ respectively. For angles $\alpha, \beta, \gamma$ we denote:
\[
R_{ZYZ}(\alpha, \beta, \gamma) := R_{Z}(\alpha) R_{Y}(\beta) R_{Z}(\gamma).
\]
\fi

\begin{Theorem}[$\mathrm{SO}(3)$-representations]
The Wigner matrix $D^{\ell}$ is a rotation matrix, to a map (also denoted $D^{\ell}$) $D^{\ell}: \mathrm{SO}(3) \rightarrow \mathrm{SO}(2\ell+1)$
\[
  \xymatrix{
    [0,2\pi] \times [0, \pi] \times [0,2\pi] \ar[rr]^{R_{ZYZ}} \ar[rd]_{D^{\ell}} & & \mathrm{SO}(3) \ar[ld]^{D^{\ell}}\\
    & \mathrm{SO}(2\ell+1) & 
  }
\]
The Winger matrix $D^{\ell}: \mathrm{SO}(3) \rightarrow \mathrm{SO}(2\ell+1)$ is a unitary $\mathrm{SO}(3)$ representation, i.e. for all $R,R'\in \mathrm{SO}(3)$ we have:
\[
D^{\ell}(RR') = D^{\ell}(R)D^{\ell}(R'), \ \ D^{\ell}(I) = I.
\]
The irreducible representation of $\mathrm{SO}(3)$ are given by the Wigner matrices $(D^{\ell})_{\ell \in \NN}$.
\end{Theorem}


\begin{Theorem}[Rotation of spherical harmonics]
For any rotation $R \in \mathrm{SO}(3)$ and any $\ell \in \NN$ we have:
\[
D^{\ell}(R)Y^{\ell}(x) = Y^{\ell}(Rx).
\]
\end{Theorem}


\begin{Theorem}[Hilbert basis of $L^2(\mathrm{SO}(3))$]
The Wigner matrix coefficients form a Hilbert basis of the the Hilbert space of square integrable functions on $\mathrm{SO}(3)$ for its Haar measure, that is: 
\begin{enumerate}
    \item For all $\ell,m,n$ and $\ell',m',n'$ such that the coefficients $D^{\ell}_{mn}$ and $D^{\ell'}_{m'n'}$ are defined we have:
\[
\int_{R} \hspace{-1mm} (D_{mn}^{\ell}D_{m'n'}^{\ell'})(R) \mathrm{d}R 
=
\hspace{-1mm}
\int_{0}^{2\pi} \hspace{-3mm}\int_{0}^{\pi}
\hspace{-2mm}\int_{0}^{2\pi}
\hspace{-3mm}
(D_{mn}^{\ell}D_{m'n'}^{\ell'})(\alpha, \beta, \gamma) \sin(\beta)\mathrm{d}\alpha \mathrm{d}\beta \mathrm{d}\gamma 
=
\delta_{\ell\ell'}\delta_{mm'}\delta_{nn'}.
\]
\item For any square integrable function $f:\mathrm{SO}(3) \rightarrow \RR$ uniquely decomposes in the Wigner basis, i.e. for all $R \in \mathrm{SO}(3)$:
\[
f(R) = \sum_{\ell \geqslant 0} \langle f^{\ell}, D^{\ell}(R)\rangle
\]
where for each $\ell \in \NN$, $f^{\ell} \in \RR^{(2\ell+1, 2\ell+1)}$ is the matrix of coefficients of $f$ associated with $D^{\ell}$.
\item Furthermore the coefficient matrices of $f$ satisfy the equivariance relation $(R.f)^{\ell} = D^{\ell}(R)f^{\ell}$ for all $\ell \in \NN, R\in \mathrm{SO}(3)$, where $(R.f)(x) := f(R^{-1}x)$. 

\end{enumerate}




 
\label{th:so3_hilbert_basis}
\end{Theorem}


\subsubsection{Decomposing products of spherical harmonics \& Wigner matrices}

\begin{Definition}[Clebsch-Gordan coefficients]
The Clebsch-Gordan coefficients are defined for any $\ell,\ell' \in \NN$, $m \in \llbracket -\ell, \ell \rrbracket, m' \in \llbracket -\ell, \ell \rrbracket$ and $L \in \llbracket |\ell-\ell'|, \ell+\ell' \rrbracket$ such that $\ell \geqslant \ell'$ and $M \in \NN$ by:
\[
\begin{aligned}
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle 
\\
:= \ 
&\delta_{M,m+m'} \sqrt{\frac{(2L+1)(L+\ell-\ell')!(L-\ell+\ell')!(\ell+\ell'-L)!}{(\ell+\ell'+L+1)!}}\ \times \\
&\sqrt{(L+M)!(L-M)!(\ell-m)!(\ell+m)!(\ell'-m')!(\ell'+m')!}\ \times \\
&\sum_k \frac{(-1)^k}{k!(\ell+\ell'-L-k)!(\ell-m-k)!(\ell'+m'-k)!(L-\ell'+m+k)!(L-\ell-m'+k)!}.
\end{aligned}
\]
The definition extends to $M < 0$ and $\ell < \ell'$ using the relations:
\[
\begin{aligned}
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle := (-1)^{L-\ell-\ell'}\langle \ell,\ell';-m,-m'|\ell,\ell';L,-M\rangle
\\
&
\langle \ell,\ell';m,m'|\ell,\ell';L,M\rangle := (-1)^{L-\ell-\ell'} \langle \ell',\ell;m',m|\ell',\ell;L,M\rangle
\end{aligned}
\]
For convenience we define the sparse tensors $Q^{L, (\ell,\ell')} \in \RR^{(2L+1)\times (2\ell+1) \times (2\ell'+1)}$ and its transpose \newline $Q^{(\ell,\ell'),L} \in \RR^{(2\ell+1) \times (2\ell'+1) \times (2L+1)}$ by:
\[
Q^{(\ell,\ell'), L} := (C^{\ell} \otimes C^{\ell'}) \Tilde{Q}^{(\ell,\ell'), L} (C^{\ell})^*, \ \
Q^{L, (\ell,\ell')} :=  C^{\ell} \Tilde{Q}^{L, (\ell,\ell')}  ((C^{\ell})^* \otimes (C^{\ell'})^*)
\]
Where the tensors $\Tilde{Q}^{L, (\ell,\ell')}$ and $\Tilde{Q}^{L, (\ell,\ell'), L}$ are sparse tensors whose non zero coefficients are given by the Clebsch-Gordan coefficients:
\[
\Tilde{Q}^{(\ell,\ell'), L}_{m, m', m+m'} := \Tilde{Q}^{L, (\ell,\ell')}_{m+m', m, m'} := \langle \ell,\ell'; m,m' | \ell,\ell'; L, \left(m + m'\right) \rangle.
\]


\iffalse
\[
Q^{L, (\ell,\ell')}_{m+m'+L, (2\ell'+1)(m+\ell) + m'+\ell'} = \langle \ell,\ell'; m,m' | \ell,\ell'; L, \left(m + m'\right) \rangle.
\]
\fi
\end{Definition}

\begin{Theorem}[Orthogonality relation of Clebsch-Gordan coefficients]
For any $\ell, \ell' \in \NN$ and $L \in \llbracket |\ell - \ell'|, \ell + \ell' \rrbracket$ we have:
\[
\sum_{L = |\ell-\ell'|}^{\ell+\ell'} Q^{(\ell, \ell'), L} Q^{L, (\ell, \ell')} = I_{(2\ell+1)(2\ell'+1)}, \ \ Q^{L, (\ell, \ell')} Q^{(\ell, \ell'),L'} = \delta_{L,L'} I_{2L+1}
\]
\end{Theorem}

\begin{Theorem}[Decomposition of spherical harmonics \& Wigner products]
\label{th:clebsh_gordan_decomposition}
For any $\ell, \ell' \in \NN$ and $L \in \llbracket |\ell - \ell'|, \ell + \ell' \rrbracket$ we have:
\[
\begin{aligned}
&
Y^{\ell} \otimes Y^{\ell'} = \sum_{L=|\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}Y^L, \ \ \ Y^L = Q^{L,(\ell, \ell')} (Y^{\ell} \otimes Y^{\ell'})
\\
&
D^{\ell} \otimes D^{\ell'} = \sum_{L=|\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}D^LQ^{L, (\ell, \ell')}, \ \ \ D^L = Q^{L,(\ell, \ell')} (D^{\ell} \otimes D^{\ell'}) Q^{(\ell, \ell'), L}.
\end{aligned}
\]
\iffalse
\[
Y^{\ell}_m Y^{\ell'}_{m'} = \sum_{L = |\ell - \ell'|}^{\ell+\ell'} Q^{(\ell, \ell'),L}_{M,m,m'} Y^{L}_M
\]
\fi
\end{Theorem}


\subsection{Steerable kernels}

\begin{Definition}[3D steerable kernel basis]
A $3D$ steerable kernel basis $\kappa$ is a finite dimensional basis of functions $\kappa_{rm}^{\ell}: \RR^3 \rightarrow \RR$ of the form:
\[
\kappa_{rm}^{\ell}(x) := \varphi_{r}^{\ell}(\Vert x \Vert_2^2) Y^{\ell}_m(x), \ \ \forall x \in \RR^3.
\]
where $\varphi_{r}^{\ell}: \RR \rightarrow \RR$ is the radial component, and the angular component is given by spherical harmonics. 
\end{Definition}
A typical choice for the radial component $\varphi_r$ is normalized Gaussian shell functions of the form:
\[
\varphi_r(t) := \frac{1}{t^{\ell / 2}} \exp \left( \frac{(\sqrt{t} - \rho_r^{\ell})^2}{2(\sigma_r^{\ell})^2}\right)
\]
where $\rho_r^{\ell}$ is the radius of the shall and the standard deviation parameter $\sigma_r^{\ell}$ controls its width. The $\frac{1}{t^{\ell / 2}}$ factor is normalizing the spherical harmonic component, as spherical harmonics are homogeneous polynomials we can normalize the input to the spherical harmonics instead. In this work we consider steerable kernels given by the Zernike basis (defined below) which also forms a Hilbert basis of the Hilbert space $L^{2}(\mathcal{B}_3)$ of square integrable functions on the unit ball $\mathcal{B}_3 \subset \RR^3$.

\begin{Definition}[Zernike polynomials (radial)]
For all $\ell, n \in \NN$ such that $n - \ell \geqslant 0$ and $2 | (n - \ell)$ the (radial) Zernike polynomial $R_{n}^{\ell}$ is a degree $k = (n - \ell) / 2$ polynomial function on the real line defined for all $x \in \RR$ by:
\[
R_{n}^{\ell}(x) = \sum_{v=0}^k R_{n,v}^{\ell} x^v
\]
whose coefficient $R_{n,v}^{\ell}$ is given by:
\[
R_{n,v}^{\ell} :=
\frac{(-1)^k}{2^{2k}} \sqrt{\frac{2\ell + 4k + 3}{3}} \begin{pmatrix}
2k \\
k
\end{pmatrix}
(-1)^v
\frac{
\begin{pmatrix}
k \\
v
\end{pmatrix}
\begin{pmatrix}
2(k+\ell+v)+1 \\
2k
\end{pmatrix}}{\begin{pmatrix}
k+\ell+v \\
k
\end{pmatrix}}.
\]
\end{Definition}

\begin{Theorem}[Orthogonality of (radial) Zernike polynomials]
For all $\ell \in \NN$ the type $\ell$ (radial) Zernike polynomials form an orthogonal family for the push forward of Lebesgue's volume measure on the unit ball to the unit interval $[0, 1[$ by the norm function. More precisely, for all $\ell \in \NN$ and all $n,n'\in \NN$ such that $n,n' \geqslant \ell$ and $2|(n-\ell)$, $2|(n'-\ell)$ we have:
\[
\int_{r=0}^1 R_n^{\ell}(r)R_{n'}^{\ell}(r) r^2 \mathrm{d}r = 
\delta_{n,n'}.
\]
\end{Theorem}

\begin{Definition}[3D Zernike polynomials]
For any $\ell,n,m$ such that $n - \ell \geqslant 0$, $2|(n-\ell)$ and $m \in \llbracket -\ell, \ell \rrbracket$ the 3D Zernike polynomial $Z^{\ell}_{nm}$ is a degree $n$ polynomial functions over $\RR^3$ defined for all $(x,y,z) \in \RR^3$ by:
\[
Z^{\ell}_{nm}(x,y,z) := R_n^{\ell}(x^2 + y^2 + z^2)Y_m^{\ell}(x,y,z).
\]
\end{Definition}

\begin{Theorem}[Hilbert basis of $L^2(\mathcal{B}_3)$]
The 3D Zernike polynomials, form a Hilbert basis of the Hilbert space $L^2(\mathcal{B}_3)$ of square integrable functions on the unit ball $\mathcal{B}_3 \subset \RR^3$, that is, for any $n,\ell,m$ and $n',\ell',m'$ such that the Zernike polynomials $Z_{nm}^{\ell}$ and $Z_{n'm'}^{\ell'}$ are defined we have:
\[
\frac{3}{4\pi}\int_{x \in \mathcal{B}_3} Z_{nm}^{\ell}(x)Z_{n'm'}^{\ell'}(x) \mathrm{d}x
=
\delta_{nn'} \delta_{\ell\ell'} \delta_{mm'}.
\]
\end{Theorem}

==> non_linearities.tex <==
\section{TFNs and equivariance to $\mathrm{SO}(3)$ subgroups}
\label{sec:eq_subgroups}



In this section we list different equivariant constructions based on $\mathrm{SO}(3)$-equivariant features as defined in \cref{def:so3_eq_feature} in particular we show how we can achieve equivariance to subgroups of $\mathrm{SO}(3)$. 

\begin{Definition}[$\mathrm{SO}(2)$-equivariant features]
A type $0$ $\mathrm{SO}(2)$-equivariant feature is a map $v^0:\RR^{N \times 3} \rightarrow \RR$ which is invariant to rotations. A type $k>0$ $\mathrm{SO}(2)$-equivariant feature of axis $\Vec{n} \in \mathcal{S}_2$ is a map $v^k:\RR^{N \times 3} \rightarrow \RR^2$ such that for all angle $\theta$:
\[
v^k(R_{\Vec{n}}(\theta).X) = e^{ik\theta}v^{k}(X).
\]
\end{Definition}


\begin{Theorem}[$\mathrm{SO}(3)$ to $\mathrm{SO}(2)$ equivariance]
Let $v$ a type $\ell$ equivariant feature, then for any $k \in \llbracket 1, \ell \rrbracket$ and any angle $\theta$ we have:
\[
v^{\ell}(R_Z(\theta).X)_{(-k,k)} = e^{ik\theta}v^{\ell}(X)_{(-k,k)}
\]
and $v^{\ell}(X)_0$ is invariant to rotations around the $Z$ axis. Furthermore for any rotation $R \in \mathrm{SO}(3)$ the feature $w^{\ell} := D^{\ell}(R) v^{\ell}$ satisfies the relation:
\[
w^{\ell}(R^{-1}R_Z(\theta)R.X)_{(-k,k)} = e^{ik\theta}w^{\ell}(X)_{(-k,k)}
\]
\end{Theorem}

\begin{Definition}[Harmonic transforms]
The harmonic transforms associated with equivariant features are defined by:
\begin{itemize}
    \item \textbf{Fourier Transform} The Fourier transform (FT) of a function $f:\mathrm{SO}(2) \rightarrow \RR$ is defined by:
    \[
    \mathcal{F}^{\ell}(f) := \int_{0}^{2\pi} f(\theta)e^{i\ell\theta} \mathrm{d}\theta
    \]
    for a discrete subset $P \subset \mathrm{SO}(2)$ we define $\mathcal{F}^{\ell}_P(f)$ by replacing the Haar measure of $\mathrm{SO}(2)$ by $\sum_{p \in P} \delta_{p}$. 

    \item \textbf{Spherical Harmonics Transforms} The Spherical Harmonics Transform (SHT) of a function $f:\mathcal{S}_2 \rightarrow \RR$ is defined by:
    \[
    \mathcal{S}^{\ell}(f) := \int_{\mathcal{S}_2} f(\theta)Y^{\ell}(x) \mathrm{d}x
    \]
    for a discrete subset $P \subset \mathcal{S}_2$ we define $\mathcal{S}^{\ell}_P(f)$ by replacing the surface measure of $\mathcal{S}_2$ by $\sum_{p \in P} \delta_{p}$. 
    
    
    \item \textbf{Wigner Transform} The Wigner Transform (WT) of a function $f:\mathrm{SO}(3) \rightarrow \RR$ is defined by:
    \[
    \mathcal{X}^{\ell}(f) := \int_{\mathrm{SO}(3)} f(\theta)D^{\ell}(R) \mathrm{d}R
    \]
    for a discrete subset $P \subset \mathrm{SO}(3)$ we define $\mathcal{W}^{\ell}_P(f)$ by replacing the Haar measure of $\mathrm{SO}(3)$ by $\sum_{p \in P} \delta_{p}$.
\end{itemize}

\begin{itemize}
    \item \textbf{Inverse FT} The inverse Fourier transform of a collection of $\mathrm{SO}(2)$-equivariant features $(v^{\ell})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ is the map $\mathcal{F}^{-1}(v): \RR^{N\times 3} \times \mathrm{SO}(2) \rightarrow \RR$ defined by:
    \[
    \mathcal{F}^{-1}(v)(X,x)
    :=
    v^{0}(X) + \sum_{\ell=1}^{\ell_{\max}} \langle v^{\ell}(X), e^{i\ell\theta} \rangle.
    \]
    \item \textbf{Inverse SHT} The inverse spherical harmonics transform of a collection of $\mathrm{SO}(3)$-equivariant features $(v^{\ell})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ is the map $\mathcal{S}^{-1}(v): \RR^{N\times 3} \times \mathcal{S}_2 \rightarrow \RR$ defined by:
    \[
    \mathcal{S}^{-1}(v)(X,x)
    :=
    \sum_{\ell=0}^{\ell_{\max}} \langle v^{\ell}(X), Y^{\ell}(x) \rangle.
    \]
    \item \textbf{Inverse WT} The inverse Wigner transform of a collection of $\mathrm{SO}(3)$-equivariant matrices $(v^{\ell}: \RR^{N \times 3} \rightarrow \RR^{(2\ell+1, 2\ell+1)})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ is the map $\mathcal{S}^{-1}(v): \RR^{N\times 3} \times \mathrm{SO}(3) \rightarrow \RR$ defined by:
    \[
    \mathcal{W}^{-1}(v)(X,R)
    :=
    \sum_{\ell=0}^{\ell_{\max}} \langle v^{\ell}(X), D^{\ell}(R) \rangle.
    \]
\end{itemize}

\end{Definition}

\begin{Theorem}[Spherical harmonics non linearities]
Let $(v^{\ell})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ a collection of equivariant features, their inverse spherical harmonic transform is defined by
\[
\mathcal{S}^{-1}(v(X))(x)
:=
\sum_{\ell=0}^{\ell_{\max}} \langle v^{\ell}(X), Y^{\ell}(x) \langle
\]
\end{Theorem}

\begin{Lemma}
Let $f: \mathrm{SO}(3) \rightarrow \RR$ then for any $R \in \mathrm{SO}(3)$ we have $(R.f)^{\ell} = D^{\ell}(R)$, where $R.f(x) := f(R^{-1}x)$.
\end{Lemma}
\begin{proof}

\end{proof}

\begin{Theorem}[Harmonic transform non linearities]
Let $\xi : \RR \rightarrow \RR$ we have:
\begin{itemize}
    \item Given a collection of $\mathrm{SO}(2)$-equivariant features $(v^{\ell})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ of axis $\Vec{n}$, then for all $\ell \geqslant 0$ $\mathcal{F}^{\ell} \circ \xi \circ \mathcal{F}^{-1}(v)$ is a type $\ell$ $\mathrm{SO}(2)$-equivariant feature of axis $\Vec{n}$. And for any finite subgroup $G \subset \mathrm{SO}(2)$, $\mathcal{F}^{\ell}_G \circ \xi \circ \mathcal{F}^{-1}(v)$ satisfies the following equivariance property for all $g \in G$:
    \[
    \mathcal{F}^{\ell}_G \circ \xi \circ \mathcal{F}^{-1}(v)(R_{\Vec{n}}(g).X)
    =
    e^{i\ell g}\mathcal{F}^{\ell}_G \circ \xi \circ \mathcal{F}^{-1}(v)(X)
    \]
    
    

    \item Given a collection of $\mathrm{SO}(3)$-equivariant features $(v^{\ell})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$, then for all $\ell \geqslant 0$ $\mathcal{S}^{\ell} \circ \xi \circ \mathcal{S}^{-1}(v)$ is a type $\ell$ $\mathrm{SO}(3)$-equivariant feature. And for any finite subset $S \subset \mathcal{S}_2$, $\mathcal{S}^{\ell}_G \circ \xi \circ \mathcal{S}^{-1}(v)$ satisfies the following equivariance property for all $R \in \mathrm{Sym}(S)$:
    \[
    \mathcal{S}^{\ell}_S \circ \xi \circ \mathcal{S}^{-1}(v)(R.X)
    =
    D^{\ell}(R)\mathcal{S}^{\ell}_S \circ \xi \circ \mathcal{S}^{-1}(v)(X)
    \]
    
    
    \item Given a collection of $\mathrm{SO}(3)$-equivariant features matrices $(v^{\ell}: \RR^{N \times 3} \rightarrow \RR^{(2\ell+1, 2\ell+1)})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$, then for all $\ell \geqslant 0$ $\mathcal{S}^{\ell} \circ \xi \circ \mathcal{W}^{-1}(v)$ is a type $\ell$ $\mathrm{SO}(3)$-equivariant feature matrix. And for any finite subgroup $G \subset \mathrm{SO}(3)$, $\mathcal{W}^{\ell}_G \circ \xi \circ \mathcal{W}^{-1}(v)$ satisfies the following equivariance property for all $g \in G$::
    \[
    \mathcal{W}^{\ell}_G \circ \xi \circ \mathcal{W}^{-1}(v)(R.X)
    =
    D^{\ell}(R)\mathcal{W}^{\ell}_G \circ \xi \circ \mathcal{W}^{-1}(v)(X)
    \]
\end{itemize}
\end{Theorem}

==> trash.tex <==
Tensor Field Networks (TFN) introduced in \Adrien{CITE} propose a different approach to equivariance compared to the methods we have presented so far. Multi view CNNs \Adrien{ref} achieve equivariance by considering all rotations of the input of a regular $\RR^3$-CNN, $\mathrm{SE}(3)$-CNNs are based on $\mathrm{SE}(3)$ convolution which are naturally $\mathrm{SE}(3)$-equivariant by construction. We have shown \Adrien{ref} that $\mathrm{SE}(3)$ are equivalent to multi view networks with cross view communication / aggregation given by $\mathrm{SO}(3)$-convolution. TFN approach $\mathrm{SE}(3)$-equivariance by starting from a regular $\RR^3$-CNN which are $\RR^3$ equivariant. The question underlying TFN construction is: What properties of kernels and weights are required to extend $\RR^3$-equivariance to $\mathrm{SE}(3)$-equivariance ? A first observation is that the $\mathrm{SO}(3)$-equivariance properties of steerable kernel bases transfer to convolutional features and linear combination of equivariant features are still equivariant features. The next question is how to stack convolutions by steerable kernels while maintaining the same equivariance properties. We now describe the TFN construction 
Given 



\section{Modeling $\mathrm{SE}(3)$-conv with Tensor Field Networks}
\label{sec:tfn}
Tensor Field Networks (TFN) operate on 3D pointcloud data, it can be extended to voxel data by by viewing it as pointcloud where each voxel is a point in 3D. TFNs are based on steerable convolution layers. In this section we show how $\mathrm{SE}(3)$ convolution can be modeled using TFN steerable convolution layers. So far we only described continuous convolutions, however TFN convolution layers are based on discretized convolutions over pointclouds. We first recall the definition of point cloud convolution and establish convenient formalism before establishing the relation between TFN conv layers and $\mathrm{SE}(3)$ convolution. A pointcloud is represented as a matrix $X \in \RR^{N \times 3}$ where $N$ is the number of points and a function over $X$ is represented by a vector $f \in \RR^N$ we recall the definition of the Point cloud convolution over a point over $X$ between $f$ and a kernel $\kappa: \RR^3 \rightarrow \RR$ is the function over $X$ defined by: 
\begin{equation}
f \ast_X \kappa_i
:=
\sum_{j = 0}^{N-1} f_j \kappa(X_i - X_j).
\label{eq:pointcloud_conv}
\end{equation}
Note that we can reformulate the above definition as a convolution over $\RR^3$ by extending the function $f$ to $\RR^3$ by setting its value outside the pointcloud to $0$ and replacing Lebesgue's measure by the sum of Dirac measures over $X$: $\delta_X := \sum_i \delta_{X_i}$, this gives:
\[
f \ast_X \kappa(x) 
:=
\int_{\RR^3} f(t) \kappa(x-t) \mathrm{d}\delta_X(t)
\]
note that the resulting function is defined over $\RR^3$ but it takes non zero values only over the pointcloud $X$ and its values on $X$ are consistent with \cref{eq:pointcloud_conv}. We extend the definition to functions over $X \times \mathrm{SO(3)} \subset \mathrm{SE}(3)$. The convolution $f \ast_X \kappa$ of a function $f$ over $X \times \mathrm{SE}(3)$ by a kernel $\kappa: \mathrm{SE}(3) \rightarrow \RR$ is defined by extending $f$ to $\mathrm{SE}(3) = \RR^3 \times \mathrm{SO}(3)$ by setting its values to $0$ outside $X \times \mathrm{SO}(3)$ and setting the measure $\lambda$ as $\delta_X := \sum_i \delta_{X_i}$ instead of the Lebesgue's measure in \cref{eq:se3_conv} i.e.:
\begin{equation}
    f \ast_X \kappa(x, R) 
    :=
    \int_{\RR^3}  \int_{\mathrm{SO}(3)} f(t,H)g(H^{-1}(x-t), H^{-1}R) d\mu(H) d\delta_X(t)
\end{equation}
Similarly for kernels $\kappa_1: \RR^3 \rightarrow \RR$ and $\kappa_2: \mathrm{SO}(3) \rightarrow \RR$ we define $f \ast_X (\delta_0 \otimes \kappa_2)$ and $f \ast_X (\kappa_1 \otimes \delta_I)$ by setting $\lambda = \delta_X$ in \cref{eq:sep_conv_1} and \cref{eq:sep_conv_2} as noted at the beginning of \cref{sec:se3_conv} all the results we have established so far hold still hold when replacing the the Lebesgue's measure of $\RR^3$ by $\delta_X$.

\paragraph{Notations} We introduce some convenient notations for indexing tensors:
\begin{itemize}
    \item For any tuples $a,b \in \ZZ^n$ we denote $\llbracket a, b \rrbracket := \prod_i \llbracket a_i, b_i \rrbracket$, if either $a$ or $b$ is replaced by an integer it is understood at the constant tuple with all entries equal to this integer. We refer to an element of $\llbracket a, b \rrbracket$ as multi-index, generalizing integer indices.
    \item For any tuples $p_1, \dots, p_k$ we denote $p_1. \dots .p_k$ their concatenation.
    \item For any tuple $p \in \NN^n$ we denote by $\RR^p$ the space of real valued tensors of shape $p$.
    \item Given positive integers tuples $p, q, r$ and tensors $W \in \RR^{p} \times \RR^q$ and $X \in \RR^{r.p}$ we denote by $X.W \in \RR^{r.q}$ the tensor defined for any multi-indices $i \in \llbracket 0, q-1\rrbracket$, $j \in \llbracket 0, q-1\rrbracket$ and $k \in \llbracket 0, r-1\rrbracket$ by:
    $
    (X.W)_{ki} := \sum_{k \in \llbracket 0, p \rrbracket} X_{kj}W_{(j,i)}.
    $
\end{itemize}



\begin{Definition}[TFN Convolution \& linear layers]
A TFN convolution layer operates over a point cloud $X$, it takes as input $(f^{\ell}: X \rightarrow \RR^{(2\ell+1).p^{\ell}})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ a collection of tensor valued signals over $X$ and a steerable kernel basis $(\kappa^{\ell}_{nm})_{\ell m n}$. For any integer $L \geqslant 0$ we denote by $I(L) := \{ (\ell, \ell') \in \NN^2 \ \vert \ |\ell - \ell'| \leqslant L \leqslant \ell + \ell'\}$. The TFN layer starts by computing $f^{\ell}_{:,j} \ast_X \kappa^{\ell'}_n$ (for any multi-index $j \in \llbracket 0, p-1 \rrbracket$) which is a signal over $X$ taking values in $\RR^{(2\ell + 1) \times (2\ell'+1)}$ it then project it to a $2L+1$ dimensional signal $Q^{L, (\ell, \ell')} f^{\ell}_{:,j} \ast_X \kappa^{\ell'}_n$ for any $(\ell, \ell') \in I(L)$ using the Clebsch Gordan projection $Q^{L, (\ell, \ell')}$. Then, all these signals are stacked over the last axis, for a obtaining a signal of dimension $|I(L)| \times (2L+1)$ for any indices $i,j,n$:
\[
\mathrm{TFNConv}(f, \kappa)^L_{i,n,j,:} 
:= 
\bigoplus_{(\ell, \ell') \in I(L)} Q^{L, (\ell, \ell')} f^{\ell}_{ij} \ast_X \kappa^{\ell'}_n
\]
A TFN linear layer (also called intertwiner) takes a collection of tensor valued maps $(f^{\ell}: X \rightarrow \RR^{(2\ell+1).p^{\ell}})_{\ell \in \llbracket 0, \ell_{\max}\rrbracket}$ and multiplies them a collection of weight matrices $(W^{\ell} \in \RR^{p^{\ell}} \times \RR^{q^{\ell}})_{\ell \in T}$ obtaining the tensor valued maps:
\[
\mathrm{TFNLin}(f, W)^{\ell} := f^{\ell}.W^{\ell}
\]
for $\ell \in \llbracket 0, \ell_{\max}\rrbracket \cap T$. TODO : talk about the bias vector for type 0 features.
\iffalse
finally the TFN conv layer applies a learnable weights tensor $W^L$ to $\mathrm{TFN}(f, \kappa)^L$ for all $L$:
\[
\mathrm{TFN}(f, \kappa, W)^L_{:,c} := \sum_{kjn} W^L_{ckjn} \mathrm{TFN}(f, \kappa)^L_{kjn,:}.
\]
\fi
\end{Definition}


\begin{Definition}[$\mathrm{SO}(3)$-Equivariant features]
\label{def:so3_eq_feature}
A type $\ell$ $\mathrm{SO}(3)$-equivariant point cloud feature is a vector valued function $v^{\ell}: \RR^{N \times 3} \rightarrow \RR^{2\ell+1}$ of a hole pointcloud satisfying the equivariance property: 
\[
v^{\ell}(XR^{\top}) := D^{\ell}(R)v^{\ell}(X).
\]
By assembling $N$ type $\ell$ equivariant features into a matrix valued map  $f:\RR^{N \times 3} \rightarrow \RR^{N \times (2\ell+1)}$ for any pointcloud $X$ we can view the matrix $f^{\ell}(X)$ as a map from $X$ to $\RR^{2\ell+1}$ where 
$f^{\ell}(X, X_i) := f^{\ell}(X)_i$, we call such a map $f^{\ell}$ a type $\ell$ feature map. Features maps can be further be stacked into equivariant tensors maps, i.e. maps $f: \RR^{N \times 3} \rightarrow \RR^{(N).(2\ell+1).p}$ where $p \in (\NN^*)^n$ and for any multi-index $j \in \llbracket 0, p-1\rrbracket$ $f(\bullet)_{:,:,j}$ is an equivariant feature map.
\end{Definition}

The main property of tensor Fields Networks is:

\begin{Theorem}[TFN and equivariant tensors]
TFN Layers map equivariant tensor maps to equivariant tensor maps, let $f$ be a collection  of tensor features maps of types $\ell \in \llbracket 0, \ell_{\max} \rrbracket$, $\kappa$ a steerable kernel basis of types $\ell' \in \llbracket 0, \ell'_{\max}\rrbracket$ and $W$ a family of intertwiner weight matrices of types $\ell'' \in T$ we have:

\begin{enumerate}
    \item  $\mathrm{TFNConv}(f, \kappa)$  is a collection of equivraiant tensor maps of types $L \in \llbracket 0, \ell_{\max} + \ell'_{\max} \rrbracket$.
    \item $\mathrm{TFNLin}(f, W)$ is a is a collection of equivraiant tensor maps of types $L \in \llbracket 0, \ell_{\max} \rrbracket \cap T$.
\end{enumerate}

\end{Theorem}

The goal of this section is to show that $\mathrm{SE}(3)$ convolution over pointclouds can be modeled using TFN convolution layers and linear layers when choosing the appropriate weights. First we must explain how TFN inputs are related to $\mathrm{SE}(3)$ signals over a point cloud, more precisely we show that such a signal can be modeled as a TFN input. Let $f: X \times \mathrm{SO}(3) \rightarrow \RR$ as explained in \cref{eq:se3_fn_pt_decomposition} the function $f$ admits a decomposition in the Wigner basis at ant point of the point cloud $X$, i.e. for all point index $i$ and integer $\ell \geqslant 0$ there exists matrices $f^{\ell}(X_i) \in \RR^{(2\ell+1) \times (2\ell+1)}$ such that:
\[
f(X_i, R) = \sum_{\ell = 0}^{\ell_{\max}} \langle f^{\ell}(X_i), D^{\ell}(R) \rangle
\]
we assume that $f$ is bandlimited, i.e. the decomposition is bounded $0 \leqslant \ell \leqslant \ell_{\max}$. For any $\ell$, $f^{\ell}$ is a map $X$ to $\RR^{2\ell+1}$, thus the map $f$ can be viewed as a TFN conv layer input. We can now state the main result:

\begin{Theorem}[$\mathrm{SE}(3)$ convolution as TFN layers]
Let $X$ be a pointcloud, and  band limited functions $f: X \times \mathrm{SO}(3) \rightarrow \RR$ and $\theta: \mathrm{SO}(3) \rightarrow \RR$ and $\kappa$ a steerable kernel basis, then the convolutions $f \ast_X (\kappa^{\ell'}_n \otimes \delta_I)$ and $f \ast_X (\delta_0 \otimes \theta)$ can be computed by a TFN conv layer followed by a TFN linear layer and a TFN linear layer respectively. 

\end{Theorem}
\begin{proof}

We denote by $W^{ m, (\ell, \ell'), L} := \left(I_{2\ell+1} \otimes (\delta_m^{\ell'})^{\top}\right) Q^{ (\ell, \ell'), L} \in \RR^{(2\ell+1)\times(2L+1)}$ and the bloc diagonal matrix $A^{ m, L} := \bigoplus_{(\ell, \ell') \in I(L)} A^{ m, (\ell, \ell'), L}$ whose blocs are the matrices $A^{ m, (\ell, \ell'), L}$, and denote 
\[
W^{m, \ell', L}_{jlk} = \mathbb{1}_{I(L, \ell')}(l)W^{ m, (\ell, \ell'), L}_{jk}
\]
where $I(L, \ell') := \{ (\ell, l) \in I(L), l = \ell'\}$ and $\mathbb{1}_{I(L, \ell')}(l)$ is the indicator function of $I(L, \ell')$ as a subset of $I(L)$ then we have:
\[
f \ast_X (\kappa_{nm}^{\ell'} \otimes \delta_I)^L 
=
\mathrm{TFNConv}(f, \kappa)^L.W^{m, \ell', L}
\]
Furthermore we have 
$
f \ast_X (\delta_0 \otimes \theta)^L 
=
f^L.\theta^L.
$
\end{proof}

\begin{Lemma}
For any $j, j', \ell, \ell', L \in \NN$ with $|\ell - \ell'| \leqslant L \leqslant \ell + \ell'$ we have $|j - j'| \leqslant L \leqslant j + j'$ we have:
\[
Q^{(\ell, \ell'), L} Q^{L,(j, j')} = 
\]
\end{Lemma}


\iffalse
\begin{Theorem}[The Wigner Basis]
\Adrien{need to cite some ref for this th}
The Wigner matrices coefficients form a Hilbert basis of $L^{2}(\mathrm{SO}(3))$, that is:
\begin{enumerate}
    \item For all $\ell,m,n$ and $\ell',m',n'$ such that the coefficients $D^{\ell}_{mn}$ and $D^{\ell'}_{m'n'}$ are defined we have:
\[
\int_{\mathrm{SO}(3)} \hspace{-1mm} (D_{mn}^{\ell}D_{m'n'}^{\ell'})(R) \mathrm{d}\mu(R)
=
\delta_{\ell\ell'}\delta_{mm'}\delta_{nn'}.
\]
\item Any square integrable function $f:\mathrm{SO}(3) \rightarrow \RR$ uniquely decomposes in the Wigner basis, i.e. for all $R \in \mathrm{SO}(3)$:
$
f(R) = \sum_{\ell \geqslant 0} \langle f^{\ell}, D^{\ell}(R)\rangle
$
where for each $\ell \in \NN$, $f^{\ell} \in \RR^{(2\ell+1, 2\ell+1)}$ is the matrix of coefficients of $f$ associated with $D^{\ell}$.
\item Furthermore the coefficient matrices of $f$ satisfy the equivariance relation $(R.f)^{\ell} = D^{\ell}(R)f^{\ell}$ for all $\ell \in \NN, R\in \mathrm{SO}(3)$, where $(R.f)(x) := f(R^{-1}x)$. 

\end{enumerate}
\label{th:so3_hilbert_basis}
\end{Theorem}
\fi


\iffalse
In our general definition of group convolution CNN \cref{def:gcnn} non linearities consist of a point-wise application of a non linear function $\xi: \RR \rightarrow \RR$ (typically a ReLu). In \cref{th:tfn_vs_se3_conv_1} we provide the expression of the harmonic decomposition of a $\mathrm{SE}(3)$-conv layer in the Wigner basis. We now discuss how to integrate pointwise non linearities with this harmonic representation and the equivariance properties of the resulting networks. As seen in \cref{sec:tfn_vs_se3_conv} $\mathrm{SE}(3)$-CNNs (or equivalently TFN) features represent $\mathrm{SE}(3)$ functions, for all $x \in \RR^3$ (or in a pointcloud) we have the decomposition of an $\mathrm{SO}(3)$ function in the Wigner basis. However there is no closed form for general pointwise non linearities (e.g. ReLu) in this representation. Therefore we convert it to a pointwise representation via inverse Wigner Transform, apply the non linearity and convert back to Wigner coefficient with Forward Wigner Transform. We follow a similar approach to \cite{poulenard2021functional} which interprets TFN features as spherical functions.
\begin{Definition}[Wigner transform]
\label{def:wigner_transform}
The forward Wigner Transform (WT) $\mathcal{W}(f)$ of a square integrable function $f:\mathrm{SO}(3) \rightarrow \RR$ is its collection of matrices coefficients in the Wigner basis. The inverse WT of a collection of matrices $(F^{\ell} \in \RR^{(2\ell+1,2\ell+1)})_{\ell}$ whose coefficients are square sumable is the associated function over $\mathrm{SO}(3)$, that is:
\[
\mathcal{W}(f)^{\ell} 
:= 
f^{\ell} 
:=
\int_{\mathrm{SO}(3)} f(R) D^{\ell}(R) d\mu(R),
\ \ \ \
\mathcal{W}^{-1}(F)(R) := \sum_{\ell} \langle F^{\ell}, D^{\ell}(R) \rangle
\]
where $\mu$ is the volume measure of $\mathrm{SO}(3)$. This definition adapts to the discrete case of a finite sampling $G \subset \mathrm{SO}(3)$ by replacing $\mu$ by $\frac{1}{|G|}\delta_G$ where $\delta_G := \sum_{g\in G} \delta_g$.

\iffalse
and a function $f$ over $G$ we define:
\[
\mathcal{W}_G(f)^{\ell} 
:=
\frac{8\pi}{|G|}\sum_{g \in G} f(g) D^{\ell}(g),
\ \ \ \
\mathcal{W}^{-1}_G(F)(g) := \sum_{\ell} \langle F^{\ell}, D^{\ell}(g) \rangle, \ \forall g \in G
\]
\fi
\end{Definition}
\fi

\iffalse
We follow a similar idea to \Adrien{CITE} where TFN equivariant features are seen as coefficient of functions on the sphere in the spherical harmonic basis and are converted to pointwise functions on the sphere or on a finite sampling of the sphere via inverse Spherical Harmonics Transforms (SHT) so that the non linearity $\xi$ can be applied in a point-wise fashion, then the point-wise functions are converted back to equivariant features by computing their SH coefficients using forward SHT. Here we follow the same idea while operating on functions over $\mathrm{SO}(3)$ and using the Wigner Transform defined below:
\begin{Definition}[Wigner transform]
The forward Wigner Transform (WT) $\mathcal{W}(f)$ of a square integrable function $f:\mathrm{SO}(3) \rightarrow \RR$ is its collection of matrices coefficients in the Wigner basis. The inverse WT of a collection of matrices $(F^{\ell} \in \RR^{(2\ell+1,2\ell+1)})_{\ell}$ whose coefficients are square sumable is the associated function over $\mathrm{SO}(3)$, that is:
\[
\mathcal{W}(f)^{\ell} 
:= 
f^{\ell} 
:=
\int_{\mathrm{SO}(3)} f(R) D^{\ell}(R) d\mu(R),
\ \ \ \
\mathcal{W}^{-1}(F)(R) := \sum_{\ell} \langle F^{\ell}, D^{\ell}(R) \rangle
\]
where $\mu$ is the volume measure of $\mathrm{SO}(3)$. This definition adapts to the discrete case of a finite sampling $G \subset \mathrm{SO}(3)$ by replacing $\mu$ by $\frac{8\pi}{|G|}\delta_G$ where $\delta_G := \sum_{g\in G} \delta_g$.

\iffalse
and a function $f$ over $G$ we define:
\[
\mathcal{W}_G(f)^{\ell} 
:=
\frac{8\pi}{|G|}\sum_{g \in G} f(g) D^{\ell}(g),
\ \ \ \
\mathcal{W}^{-1}_G(F)(g) := \sum_{\ell} \langle F^{\ell}, D^{\ell}(g) \rangle, \ \forall g \in G
\]
\fi
\end{Definition}

\begin{Theorem}[Equivariance of non linearities]
The network defined by: 
\[
F(f,W) := y^n(f), \ y^{k+1}(f) := \mathcal{F} \circ \xi \circ \mathcal{F}^{-1}(\mathrm{Conv}_{\mathrm{SE}(3)}(y^{k}(f), W^{k+1})), \ y_0 := f
\]
is a standard $\mathrm{SE}(3)$-CNN if $\mathcal{F} = \mathcal{W}$ is the Wigner transform. If $\mathcal{F} = \mathcal{W}_G$ where $G \subset \mathrm{SO}(3)$ is a finite subgroup then $F$ is equivariant to $G$, i.e. for all $R \in G$ we have 
$F(R.f, W)^{\ell} = D^{\ell}(R)F(f, W)^{\ell}$.
\end{Theorem}
\fi
